Optimization-Based Resiliency Verification in Microgrids via Maximal Adversarial Set Characterization

Critical energy infrastructures are increasingly relying on advanced sensing and control technologies for efficient and optimal utilization of flexible energy resources. Algorithmic procedures are needed to ensure that such systems are designed to be resilient to a wide range of cyber-physical adversarial events. This paper provides a robust optimization framework to quantify the range of adversarial perturbations that a system can accommodate without violating pre-specified resiliency metrics. An inner-approximation of the set of adversarial events which can be mitigated by the available flexibility is constructed using an optimization based approach. The proposed algorithm is illustrated on an islanded microgrid example: a modified IEEE 123-node feeder with distributed energy resources. Simulations are carried out to validate that the resiliency metrics are met for any event sampled from the constructed adversarial set for varying levels of available flexibility (energy reserves).

==> ACC_sections/scenarios.tex <==
The resiliency of energy systems (including microrgids) against various cyber and physical adversarial events, including malicious attacks, have been studied in the literature \cite{dehghani2021cyber,wang2019deep,dehghani2021blockchain,sahoo2018stealth}. One type of such attack includes injecting measurement errors to renewable generation output. Such errors can be constant offsets or potentially time-varying, and left untreated, may eventually lead to ramp-induced attacks \cite{che2019impact}. Another class of attacks include \textit{replay attacks} \cite{habibi2020detection}, whereby the measured renewable generation output is maliciously changed to reflect the true generation at a previous time stamp, thus impacting dispatch decisions. A third class of attacks entails corruption of state estimation, whereby the estimated physical quantities required for dispatch decisions (such as load setpoints) are maliciously changed \cite{kushal2018risk}, \cite{banerjee2021online}. Specifically, load-setpoint change attacks often cause maximal impact when affected during specific hours of the day (for example, during 12pm - 7pm, when load typically rises to hit an evening peak). A final class of attacks is coordinated attacks, whereby an attacker often has access to multiple critical information of the system, and can maliciously pose threats in a coordinated manner, from multiple sources (such as malicious under-estimation of load coupled with over-estimation of renewable capacity). Examples of such attacks, which often include attacks in both the cyber as well as the physical layer can be found in~\cite{sun2018cyber}, \cite{he2021tri}, \cite{che2019impact}. 
% 
In addition to malicious attacks, other physical events such as generator outage, loss of solar generation due to cloud coverage, etc., could also lead to violations of critical operational constraints (such as serviceability of critical loads) as specified in Sec.\,\ref{sec:baseline}. In the following, we describe a robust extension of \eqref{eq:baseline}.



% These can be broadly grouped into the following categories, as shown below:

% \begin{itemize}
%     \item \textbf{Injecting measurement errors into PV generation output:} Within this type of attack, we can have several possibilities:
%     \begin{itemize}
%         \item Inject $\epsilon$ error to the PV generation at all time stamps, i.e.,
%         $$\hat{S}_{n,k}^S = S_{n,k}^S\times (1+\epsilon),$$ where $\epsilon \in [-1,1]$. The factor $\epsilon$ can be tweaked to emulated systematic under-estimations as well as over-estimations.
%         %For implementation purpose, we can treat $\epsilon$ to be a parameter, and vary in discrete steps, such as $\epsilon = \{0.1, 0.2, 0.3\}$. 
%         \item Inject time-varying errors instead of static error.
%     \end{itemize}
%     These type of error, left untreated, can lead to ramp-induced attacks (RID), as discussed in details in \cite{che2019impact}.
    
%     \item \textbf{Injecting latency to PV generation output measurement (Replay attack):} In this type of attack (see, for example \cite{habibi2020detection}), the measured PV-generation output is maliciously changed to reflect the true generation at a previous time stamp (with $\delta$ delay). Mathematically, $$\hat{S}_{n,k}^S = S_{n,k-\delta}^S,$$ where $\hat{S}^S$ denotes the measured PV-generation output to be used in the microgrid optimization.
    
%     \item \textbf{Injecting errors to load measurement (corrupted state estimation):} This type of attack is also known as load curtailment cyber-attack (see \cite{kushal2018risk}, \cite{banerjee2021online} for detailed case studies). Similar to generation setpoint change attack, assuming $\epsilon$ to be the malicious error injection, we can write:
%     $$ \hat{S}_{n,k}^L = S_{n,k}^L \times (1 + \epsilon), $$
%     Note that as given in \cite{kushal2018risk}, it may be optimal for the attacker (causing maximal disruption) when this type of attack is initiated around afternoon (12 pm) and continued till peak evening hours. 
    
%     \item \textbf{Partial/complete loss of dispatchable generation capability}
    
%     \item \textbf{Coordinated attack schemes:} In this type of attack, the attacker often has access to multiple critical information of the system, and is in a position to maliciously pose threats in a coordinated manner, from multiple sources. Examples of such attacks, which often include attacks in both the cyber as well as the physical layer can be found in~\cite{sun2018cyber}, \cite{he2021tri}, \cite{che2019impact}.
%     %In our work, we consider at least 1 type of coordinated attack scheme, where the attacker can simultaneously inject error signals to load estimation as well as PV-forecast, such that load is under-estimated and PV-generation is over-estimated, so that the real time generation-load imbalance is magnified, thus upsetting real time grid operations.
% \end{itemize}
